Who's Watching You Zoom? Investigating Privacy of Third-Party Zoom Apps

Zoom serves millions of users daily and allows third-party developers to integrate their apps with the Zoom client and reach those users. So far, these apps' privacy and security aspects, which can access rich audio-visual data (among others) from Zoom, have not been scientifically investigated. This paper examines the evolution of the Zoom Marketplace over one year, identifying trends in apps, their data collection behaviors, and the transparency of privacy policies. Our findings include worrisome details about the increasing over-collection of user data, non-transparency about purposes and sharing behaviors, and possible non-compliance with relevant laws. We believe these findings will inform future privacy and security research on this platform and help improve Zoom's app review process and platform policy.

==> pets/header.tex <==
\usepackage{enumitem}

\usepackage{color}
\usepackage{soul}
% Add your packages here
\usepackage{todonotes}
\usepackage[draft,inline,nomargin]{fixme}
\usepackage{xspace}
\newcommand{\rakib}[1]{\textbf{\textcolor{orange}{[rakib says: #1]}}}
\newcommand{\mustfix}[1]{\fixme{\hl{#1}}}
\newcommand{\pleasenote}[1]{\fxnote{\hl{#1}}}
\newcommand{\hlfixme}[1]{\fixme{\hl{#1}}}
\newcommand{\hlfxnote}[1]{\fxnote{\hl{#1}}}
\newcommand{\eg}{{\it e.g.,}}
\newcommand{\ie}{{\it i.e., }}
\newcommand{\etal}{{\it et al.}}
\newcommand{\gc}[1]{\vspace{1mm}\noindent\hl{General comment: #1}}
\newcommand{\x}{\hl{XXx}\xspace}
\newcommand{\y}{\hl{YYy}\xspace}
\newcommand{\n}{\hl{(N=?)}\xspace}

\newcommand{\parX}[1]{\vspace{1mm}\noindent \textbf{#1}}

\newcounter{todocount}
\setcounter{todocount}{1}
\newcommand{\todos}[1]{{\vspace{1mm}\noindent\color{red}{ [\underline{\textbf{TODO} \#\thetodocount}: } {#1}] } \stepcounter{todocount}}
\newcommand{\done}[1]{\noindent{\color{blue} DONE: #1 }\xspace}

